MUVO: A Multimodal Generative World Model for Autonomous Driving with Geometric Representations

World models for autonomous driving have the potential to dramatically improve the reasoning capabilities of today's systems. However, most works focus on camera data, with only a few that leverage lidar data or combine both to better represent autonomous vehicle sensor setups. In addition, raw sensor predictions are less actionable than 3D occupancy predictions, but there are no works examining the effects of combining both multimodal sensor data and 3D occupancy prediction. In this work, we perform a set of experiments with a MUltimodal World Model with Geometric VOxel representations (MUVO) to evaluate different sensor fusion strategies to better understand the effects on sensor data prediction. We also analyze potential weaknesses of current sensor fusion approaches and examine the benefits of additionally predicting 3D occupancy.

==> section/4_experiments.tex <==
\subsection{Dataset}\label{subsubsec: dataset}
        \textbf{Training Set.}\label{training set} We collected a training dataset $\mathcal{{D}}_{{train}}$ in the CARLA simulation environment~\cite{Dosovitskiy17} using an expert reinforcement learning agent~\cite{zhang2021roach,huModelBasedImitationLearning2022}. Our data collection encompasses four towns (Town01, Town03, Town04, Town06) and four weather conditions (Clear Noon, Wet Noon, Hard Rain Noon, Clear Sunset), gathered at a frequency of 10~FPS. For each town, we executed 25 runs, each lasting 300 seconds, with randomly selected weather conditions, amounting to 300,000 frames of data. We obtain RBG image $\mathcal{I} \in \mathbb{R}^{3 \times 600 \times 960}$, depth map $\mathcal{I}_D \in \mathbb{R}^{1 \times 600 \times 960}$, e.g., derived from stereo cameras, point cloud $\mathcal{P} \in \mathbb{R}^{\leq60,000 \times 3}$ obtained from a lidar with 64 vertical channels, route map $route \in \mathbb{R}^{1 \times 64 \times 64}$ as the planned route in BEV space, speed $\mathbf{v} \in \mathbb{R}$, and actions $\mathbf{a} \in \mathbb{R}^2$ in the form of acceleration and steering angle.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\textwidth]{img/2D_latent.pdf}
    \caption{Two-dimensional latent space: We compare a 1D baseline to a set of 2D latent spaces, where we also examine the influence of a vision-transformer backbone and an additional perceptual loss term~(\textbf{PL}). For the backbone, we evaluate ResNet18~(\textbf{RN}) and MobileVit-V2~(\textbf{VIT}).}
    \label{fig:latent_space_voxel}
\end{figure*}

        \textbf{Validation Sets.}\label{validation set} We adopt the same setup as before for two distinct validation sets. For each town, we execute five 300-second long driving sessions with the following settings:
        
        $\mathcal{{D}}_{{val}}^{RL}$: This set uses the same cities and weather conditions as the training set. However, the driving routes are randomized. The goal is to evaluate the effectiveness of our model in representation learning (RL) in familiar environments.
        
        $\mathcal{{D}}_{{val}}^{{DS}}$: We maintain the same cities as in the training set but introduce different weather conditions. The driving routes are also randomized to evaluate the model performance under domain shifts~(DS).
        
    \subsection{Training Parameters}
        We sampled data at intervals of 0.2 seconds, creating sequences of length 12 to serve as training inputs. All 12 frames were treated as known data. In the experiments containing voxel reconstructions, we reduced the length of sequences to 6 to speed up the training. We trained with a batch size of 16 and the AdamW optimizer with a learning rate of $10^{-4}$ and a weight decay of $0.01$. For validation, we used 6/4 frames as given observations, while 6/2 served as ground truth.
